BoningKnife: Joint Entity Mention Detection and Typing for Nested NER via prior Boundary Knowledge

While named entity recognition (NER) is a key task in natural language processing, most approaches only target flat entities, ignoring nested structures which are common in many scenarios. Most existing nested NER methods traverse all sub-sequences which is both expensive and inefficient, and also don't well consider boundary knowledge which is significant for nested entities. In this paper, we propose a joint entity mention detection and typing model via prior boundary knowledge (BoningKnife) to better handle nested NER extraction and recognition tasks. BoningKnife consists of two modules, MentionTagger and TypeClassifier. MentionTagger better leverages boundary knowledge beyond just entity start/end to improve the handling of nesting levels and longer spans, while generating high quality mention candidates. TypeClassifier utilizes a two-level attention mechanism to decouple different nested level representations and better distinguish entity types. We jointly train both modules sharing a common representation and a new dual-info attention layer, which leads to improved representation focus on entity-related information. Experiments over different datasets show that our approach outperforms previous state of the art methods and achieves 86.41, 85.46, and 94.2 F1 scores on ACE2004, ACE2005, and NNE, respectively.

==> figures/compare.tex <==
\begin{table*}[ht]
\caption{Comparison between our approach (\textbf{BoningKnife}) and previous works on boundary detection to solve the nested NER problem.}
\label{tab:compare-to-other-boundary}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{sc}

\begin{tabular}{p{3.2cm}|p{4cm}|p{2.5cm}|p{2.2cm}|p{2.4cm}}
\toprule
\textbf{Model} & \textbf{Boundary Knowledge} & \textbf{Candidate set generation method} & \textbf{Can handle large spacing span?} & \textbf{Can handle low S/E probality span?}\\
\midrule
Boundary-aware \cite{zheng2019boundary} & Start + End & base on S/E & N & N \\
\hline
Boundary enhanced \cite{tan2020boundary} & Start, End & base on S/E & N & N \\
\hline
% MRC-NER \cite{li2019unified} & Start, End, Span & From \textbf{SAME} representation & base on S/E + Span & Indirect & N \\
% \hline
\textbf{BoningKnife} (this work) & Star, End, Mention, Entity token  & base on span & Y & Y \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}



==> figures/main_result_after.tex <==
\begin{table*}[!t]
   \centering
   \vskip 0.1in
%   \begin{small}
    \resizebox{\linewidth}{!}{%
   \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
   \toprule
   \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{ACE2004}} & \multicolumn{3}{c}{\textbf{ACE2005}} & \multicolumn{3}{c}{\textbf{NNE}} \\ \cmidrule(l){2-10} 
    & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\ \midrule
      %  \hline
      \citet{wang2018neural}      &78.0  & 72.4  & 75.1  &76.8  & 72.3  & 74.5 & 91.8  & 91.1  & 91.4  \\
      \citet{xia2019multi} [ELMO] &81.7  & 77.4  & 79.5  &79.0  & 77.3  & 78.2 & - & - & -  \\
      \citet{luan2019general}     &   -  &   -   & 84.7  &   -  &   -   & 82.9 & - & - & - \\
      \hline
      {BERT} merge outmost \& inmost$^{\dag}$&80.55 & 79.23 & 79.88 &78.12 & 82.71 & 80.35 & 80.43 & 74.94 & 77.59 \\
      \citet{fisher2019merge}$^{\dag}$     &   -  &   -   &   -   &82.7  & 82.1  & 82.4 & - & - & -  \\
      \citet{strakov2019neural}$^{\dag}$   &   -  &   -   & 84.4  &   -  &   -   & 84.3 & - & - & -  \\
      \citet{shibuya2019nested}$^{\dag}$   &85.23 & 84.72 & 84.97 &83.30 & 84.69 & 83.99 & 93.03  & 93.34  & 93.19 \\
      \citet{tan2020boundary}$^{\dag}$    &85.8 & 84.8 & 85.3 &83.8 & 83.9 & 83.9 & - & - & - \\
      \citet{li2019unified}[ACL2020]       &85.05 & 86.32 & \textit{85.68} \footnotemark & \textbf{87.16} & {86.59} & \textbf{86.88} & - & - & - \\
      \hline
      \textbf{BoningKnife}$^{\dag}$         &{85.98} & {86.86} & {86.41} &{84.77}  & {86.16}  & {85.46} &{93.74} & {94.75} & {94.24}  \\
      \hline
      \citet{yu-etal-2020-named}[ACL2020][BERT-Large] &  87.3 & 86.0 & 86.7 & 85.2 & 85.6 & 85.4 & - & - & - \\
      \citet{wang-etal-2020-pyramid}[ACL2020][ALBERT+BERT] & \textbf{87.71} & \textbf{87.78} & \textbf{87.74} & 85.30 & \textbf{87.40} & 86.34 & \textbf{94.30} & \textbf{95.07} & \textbf{94.68} \\
      \citet{wang-etal-2020-pyramid}[ACL2020][Basic+BERT-Large] & 86.08 & 86.48 & 86.28 & 83.95 & 85.39 & 84.66 & 93.97 & 94.79 & 94.37 \\
      \citet{fu2020nested}[AAAI2021][BERT-Large] & 86.7 & 86.5 & 86.6 & 84.5 & 86.4 & 85.4 & - & - & - \\
      \citet{Xu_Huang_Feng_Hu_2021}[AAAI2021][BERT-based] & 86.9 & 85.8 & 86.3 & 85.7 & 85.2 & 85.4 & - & - & - \\
      \citet{shen2021locate}[ACL2021][BERT-Large] & 87.44 &  87.38 & 87.41 & 86.09 & 87.27 & 86.67 & - & - & - \\
      \cite{yan2021unified}[ACL2021][BERT-Large] & 87.27 & 86.41 & 86.84 & 83.16 & 86.38 & 84.74 & - & - & - \\
    \bottomrule
   \end{tabular}%
    }
%   \end{small}
   \caption{Results of the proposed \textit{BoningKnife} and prior state-of-the-art methods over the ACE2004/2005 test sets. $^{\dag}$ denotes models utilizing $\mathrm{BERT}$. '-' denotes results not reported.}
   \label{tab:main_results}
\end{table*}
   

==> figures/phased.tex <==
\begin{table*}[htbp]
\centering
\vskip 0.1in
% \begin{small}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Subtask}} & \multicolumn{3}{c|}{\textbf{ACE2004}} & \multicolumn{3}{c|}{\textbf{ACE2005}} & \multicolumn{3}{c}{\textbf{NNE}} \\ \cmidrule(l){2-10} 
 & \textbf{P}(\%) & \textbf{R}(\%) & \textbf{F1}(\%) & \textbf{P} (\%) & \textbf{R}(\%) & \textbf{F1} (\%) & \textbf{P} (\%) & \textbf{R}(\%) & \textbf{F1} (\%) \\ \midrule
entity start & 96.95 & 97.30 & 96.97 & 96.19 & 95.31 & 95.75 & 98.78 & 98.62 & 98.70  \\
 entity end & 96.61 & 96.53 & 96.57 & 95.76 & 94.72 & 95.24 & 98.81 & 98.44 & 98.62\\
 entity detection & 95.70 & 95.72 & 95.71 & 94.83 & 93.95 & 94.39 & 98.63 & 98.27 & 98.45 \\
 SpanTagger & 89.46 & 92.04 & 90.73 & 87.72 & 91.71 & 89.67 & 95.48 & 97.56 & 96.51 \\
 \bottomrule
\end{tabular}%
% }
% \end{small}
\caption{The result of each phase in ACE2004, ACE2005, NNE three benchmarks test set.}
\label{tab:phase_resuult}
\end{table*}

